NNStreamer: Efficient and Agile Development of On-Device AI Systems

We propose NNStreamer, a software system that handles neural networks as filters of stream pipelines, applying the stream processing paradigm to deep neural network applications. A new trend with the wide-spread of deep neural network applications is on-device AI. It is to process neural networks on mobile devices or edge/IoT devices instead of cloud servers. Emerging privacy issues, data transmission costs, and operational costs signify the need for on-device AI, especially if we deploy a massive number of devices. NNStreamer efficiently handles neural networks with complex data stream pipelines on devices, significantly improving the overall performance with minimal efforts. Besides, NNStreamer simplifies implementations and allows reusing off-the-shelf media filters directly, which reduces developmental costs significantly. We are already deploying NNStreamer for a wide range of products and platforms, including the Galaxy series and various consumer electronic devices. The experimental results suggest a reduction in developmental costs and enhanced performance of pipeline architectures and NNStreamer. It is an open-source project incubated by Linux Foundation AI, available to the public and applicable to various hardware and software platforms.

==> sections/obsolete/S04_Implementation.tex <==

\textit{NNStreamer} is not an experimental prototype.
It is software developed and released for commercially available products for a wide range of types.



A few authors have been working for an autonomous vehicle project,
where the need for the stream processing paradigm has emerged.
The vehicle has a lot of heterogeneous sensors and neural networks inter-connected with complex topology, transmitting large data streams, and processed simultaneously.
The vast data transmission overhead has been the core cause requiring \textit{NNStreamer}.
Then, managing complex and ever-changing data paths, allowing different NNFWs, and parallelism have added the need further.



Spinning off from the autonomous vehicle project, we have discovered that other projects share the same issues: robots, manufacturing plants, and consumer electronics.
As a result, \textit{NNStreamer} has already had a lot of potential applications in the affiliation from the beginning, which enforces to release partial but practical solutions quickly.


\begin{quote}
    Don't reinvent the wheel, just realign it.\\
    -- Anthony J. D'Angelo
\end{quote}


If we implement yet another stream framework, it may take too much time and effort.
Fortunately, we already have a stable, widely-deployed, and open-source stream framework with rich features: GStreamer.
GStreamer is a multimedia stream framework battle-tested with services (e.g., BBC~\cite{BBCGSTCONF}) and consumer electronics (e.g., televisions of both Samsung and LG), where multimedia performance is critical.
Releasing a large number of products, they have made sure that GStreamer is reliable, high-performing, and rich-featured.
Tizen, which runs a wide range of devices including most consumer electronics~\cite{ham2019tizen}, also has GStreamer as its standard multimedia engine.
As a result, most of the requirements in Chapter~\ref{SS_OtherRequirements} and the above are already satisfied by GStreamer.



We only need to ``realign'' GStreamer for neural networks and their applications.
We implement what GStreamer is missing: the features described in Chapter~\ref{S_Approach} except for ``Tee'', ``Valve'', ``Switch'', ``Queue'', and conventional media filters.



\subsection{Standard Stream Data Types}

We define two new GStreamer data types, ``\texttt{other/tensor}'' and ``{\tt other/tensor}\textbf{s}'', representing a stream of a multidimensional array and a stream of multiple instances of such arrays with different dimensions, respectively.
Listing~\ref{lst:tensor_format} describes the two GStreamer stream types in detail. 
Note that the number of tensors in ``{\tt other/tensor}\textbf{s}'' is limited to 16 only because frame buffers of GStreamer stream may have up to 16 disjoint memory chunks by default, which we can change in build-time.
These disjoint memory chunks allow to mux and synchronize multiple streams without copying the memory chunks to transmit.
We have decided not to change such a limit because we have not yet found a case where we need to synchronize more than 16 streams simultaneously from our various product requirements.
Besides, because the GStreamer binary determines the limit at build-time, if we use GStreamer built to support more memory chunks, \textit{NNStreamer} automatically supports more tensors with ``{\tt other/tensor}\textbf{s}''.

\definecolor{mygreen}{rgb}{0,0.4,0}
\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  captionpos=b,
  commentstyle=\color{mygreen},
}
\begin{figure}
\noindent\begin{minipage}{\columnwidth}
\begin{lstlisting}[label={lst:tensor_format}, caption={Tensor stream data type definition}.]
  other/tensor
    framerate = (fraction) [0/1, 2147483647/1]
    dimension = Dim
    type = Type
  
  other/tensors
    num_tensors = [1, 16]
    framerate = (fraction) [0/1, 2147483647/1]
    dimensions = Dims
    types = Types
  # num_tensors == # types == # dimensions.

  Types = Type | Type,Types
  Type = {uint8, int8, uint16, int16, uint32,
    int32, uint64, int64, float32, float64}
  Dims = Dim | Dim,Dims
  Dim = [1,65535]:[1,65535]:[1,65535]:[1,65535]
  # [min, max]: allowed value ranges.
\end{lstlisting}
\end{minipage}
\end{figure}

Unlike other approaches~\cite{GSTCONF18_DEEPSTREAM,GSTCONF18_Intel,GSTCONF18_Pexip,GSTCONF18_RidgeRun}, neural networks of \textit{NNStreamer} do not rely on conventional media types, but the above because of the advantages mentioned in Chapter~\ref{S_Approach}.
For demonstrations, we may assume that the neural network output is a video stream; however, if an application uses the output, it usually wants the raw data, not the rasterized video frames.
More critically, if a neural network requires an output of another neural network as its input, conventional media types do not fit often; e.g., an array of label probabilities is neither audio or video.
Besides, inputs of a neural network may require different forms of the given media input types (e.g., resolutions, color formats, or framerates), or may require non-media types (e.g., locations, probabilities, and labels of objects).
Therefore, standard tensor data stream types are critically required.


\subsection{Stream Filters}

\textit{NNStreamer} offers the following elements as stream filters.

\begin{itemize}
    \item \textbf{tensor\_converter} converts audio, video, text, or arbitrary binary streams to {\tt other/tensor} streams.
    \item \textbf{tensor\_decoder} converts {\tt other/tensor(s)} to video or text stream with assigned sub-plugins.
    \item \textbf{tensor\_filter} invokes a neural network model with the given model path and NNFW name.
    \item \textbf{tensor\_transform} applies various operators to tensors including typecast, add, mul, transpose, and normalize. For faster processing, it supports SIMD instructions and multiple operators in a single filter.
    \item \textbf{tensor\_\{mux, demux, merge, split, aggregator\}} support tensor stream path controls. Although GStreamer has mux and demux elements, they do not support {\tt other\//tensors} and its synchronization policies, but support multimedia containers such as avi, mkv, and mp4; therefore, we still need new mux and demux elements.
    \item \textbf{tensor\_reposink} and \textbf{tensor\_reposrc} implement Recurrent Helper of Figure~\ref{FIG_EXPPLN_Path_RNN}. Tensor\_reposink creates a shared tensor repository and inserts tensors to the repository (input of Recurrence Helper) and tensor\_reposrc retrieves tensors from the repository (output of Recurence Helper). The pair of sink and src are matched by the property, \textit{slot-index}. A tensor\_reposrc may generate a zero-filled tensor to bootstrap the cycle. For example, in the figure, to start the pipeline, Model 1 waits for the first output of Recurrence Helper, which, in turn, waits for the first output of Model 1, which is still waiting.
    \item \textbf{tensor\_ros\_\{src, sink\}} connect with ROS~\cite{quigley2009ros} nodes.
    \item \textbf{tensor\_src\_iio} accepts arbitrary sensors with the Linux IIO subsystem as inputs.
    \item \textbf{amcsrc} accepts Android MediaCodec as inputs.
\end{itemize}



Two elements accept user-created methods in run-time: tensor\_filter and tensor\_decoder.
For tensor\_filter, we provide the following sub-plugins:
TensorFlow, TensorFlow-lite, Caffe2, PyTorch, nn-fw/cc\footnote{This is a set of neural network runtime and compiler, which intends to dissect a given neural network into sub-networks so that we can utilize all of CPU, GPU, and NPU simultaneously in an embedded device. It is available at \url{https://git.tizen.org/cgit/platform/core/ml/nnfw/}}, Movidius-NCSDK2, and wrappers for general programming languages (C/C++ and Python2/3) as ``custom'' filters. 
For tensor\_decoder, we provide ``bounding-boxes'', ``imagelabel'', ``imagesegment'', and ``pose'' sub-plugins.
Developers may implement their sub-plugins quickly with the given code-gen and templates and attach them in run-time.


\begin{figure}[tb]
\begin{center}
\includegraphics[width=0.98\columnwidth]{figures/FIG_IMPL_SUBPLUGIN.png}
\end{center}
\caption{User sub-plugins (shaded) applied to elements}
\label{FIG_IMPL_SUBPLUGIN}
\end{figure}

% Experimental Environment
\begin{table*}[ht]
    \centering
    \begin{tabular}{l c c c c}
         & \texttt{A} / Artik 530s & \texttt{B} / Odroid-XU4 & \texttt{C} / 8890 & \texttt{D} / PC\\
         &&&&\vspace{-1em}\\
         \hline
         &&&&\vspace{-1em}\\
    SoC  & Nexell S5P4418 & Samsung Exynos 5422 & Samsung Exynos 8890 & Intel i7-7700 \\
         &&&&\vspace{-1em}\\
    ISA  & armv7 (32 bits) & armv7 (32 bits) & armv8 (64 bits) & x64 (64 bits) \\
         &&&&\vspace{-1em}\\
    CPU Microarchitecture & 4 CA9 & 4 CA15 + 4 CA7 & 4 Mongoose + 4 CA53 & 4 Kaby-Lake\\
         &&&&\vspace{-1em}\\
    CPU Clock Speed & 1.2 GHz & 2 GHz / 1.5GHz & 2.3 GHz / 1.6 GHz & 3.6 GHz \\
         &&&&\vspace{-1em}\\
    DRAM Capacity & 1~GiB DDR3 & 2~GiB LPDDR3 & 4~GiB LPDDR4 & 16~GiB DDR4\\
         &&&&\vspace{-1em}\\
    DRAM Throughput%
    \footnotemark
    & {0.51 / 0.75} & {2.62 / 4.08} &  {5.86 / 6.40} & {18.54 / 13.78}\\
         &&&&\vspace{-1em}\\
    OS \& Linux Kernel & Ubuntu 16.04 / 4.4 & Tizen 5.0 / 4.1 & Tizen 5.0 / 3.18 & Ubuntu 16.04 / 4.15 \\
         \hline
    \end{tabular}
    \caption{Specification of experimented devices. CA denotes Cortex-A. Linux kernels are supplied by the vendors.}
    \label{TBL_SPEC_BOARDS}
\end{table*}

Figure~\ref{FIG_IMPL_SUBPLUGIN} shows how user-created neural networks and decoders can be attached to tensor\_filter and tensor\_decoder in a pipeline.
In the figure, ``{\tt make3DBoxes.so}'' is a neural network without NNFWs and ``{\tt 3dboxdraw.so}'' is a user decoder sub-plugin, decoding results of ``{\tt make3DBoxes.so}'' to video streams.
Instead, if the tensor\_filter element has ``{\tt mode=\ tensor\-flow-\-lite}'' and ``{\tt model=x.tflite}'', TensorFlow-lite processes ``{\tt x.tflite}''.




%\begin{figure}[tb]
%\begin{center}
%\includegraphics[width=0.95\columnwidth]{figures/FIG_TRACING_11.png}
%\end{center}
%\caption{Screenshot of profiling an \textit{NNStreamer} pipeline. The highlighted filter has consumed 57.8 s of CPU time, which is 98.5\% of the whole pipeline's consumption and 88.4\% of CPU utilization during the test run.}
%\label{FIG_IMPL_TRACE}
%\end{figure}


\subsection{Developmental Environments}

We provide APIs in C, C\#, and Java, integrated with Tizen Studio and Android Studio.
Tizen Studio supports \textit{NNStreamer} APIs natively since Tizen 5.5 M2 (October 2019).
Android Studio supports \textit{NNStreamer} APIs via JCenter.
GStreamer has its APIs, which expose the full capability of \textit{NNStreamer}; however, they expose too many features and are overkill for most applications.
\textit{NNStreamer} APIs are more straightforward and provide privilege restrictions and controls for its software platforms.


A CI system~\cite{TAOS-CI} tests every code change in the \textit{NNStreamer} code repository with test cases, applications, and static analyzers for multiple hardware and software platforms. This system ensures the integrity of \textit{NNStreamer} with the contributions from the public.





% ######## Instruction manual
% https://github.sec.samsung.net/STAR/NNStreamer/tree/master/tools/profiling
%
% ######## Example script
% $ gst-launch-1.0 textoverlay name=overlay font-desc="Sans, 26" ! \
%    videoconvert ! ximagesink name=img_test \
%    v4l2src name=cam_src ! videoscale ! video/x-raw,width=640,height=480,format=RGB ! \
%    tee name=t_raw \
%    t_raw. ! queue ! overlay.video_sink \
%    t_raw. ! queue ! videoscale ! video/x-raw,width=224,height=224 ! \
%    tensor_converter ! \
%    tensor_filter framework=tensorflow-lite \
%    model=tflite_model/mobilenet_v1_1.0_224_quant.tflite ! \
%    tensor_decoder mode=image_labeling \
%    option1=tflite_model/labels.txt ! \
%    overlay.text_sink
% 
% ######## Output
% $ gst-report-1.0  pipeline0.gsttrace
% ELEMENT           %CPU   %TIME   TIME
% tensorfilter0      88.4   98.5    57.8 s
% videoscale0         0.8    0.9    524 ms
% overlay             0.2    0.3    154 ms
% videoscale1         0.1    0.1   67.3 ms
% videoconvert0       0.1    0.1   64.8 ms
% img_test            0.0    0.0   16.4 ms
% t_raw               0.0    0.0   16.1 ms
% queue0              0.0    0.0   10.6 ms
% capsfilter0         0.0    0.0   5.52 ms
% tensordec0          0.0    0.0   4.18 ms
% queue1              0.0    0.0   2.66 ms
% tensorconverter0    0.0    0.0   1.72 ms
% capsfilter1         0.0    0.0   1.10 ms
% cam_src             0.0    0.0    370 us
% pipeline0           0.0    0.0      0 ns
% 
% ######### Original source
% \\10.113.111.238\swcsait\papers\tool-tracing-data-figure
%


%We can reuse a wide range of stream analysis tools including profilers, tracers, test suites, and debuggers from GStreamer.
%Figure~\ref{FIG_IMPL_TRACE} is a screenshot of a tool analyzing a \textit{NNStreamer} pipeline.
%We heavily depend on such tools to optimize or to fix bugs of commercialization projects.




==> sections/obsolete/S06_FutureWork.tex <==

We have the following work-in-progress features not discussed in this paper.
We plan to support Protocol Buffers~\cite{PROTOBUF} and FlatBuffers~\cite{FLATBUF} as transport layers for distributed nodes and if-then-else expressions for stream path controls.
We are also implementing additional sub-plugins of \textbf{tensor\_filter} to support Keras, openVINO, edge-TPU, and more AI hardware accelerators.



There are long-term plans, as well.
We will apply the actor model~\cite{agha1985actors} to make pipelines fully-distributed.
Robotics projects often incur multiple nodes with different roles,
which requires distributes pipelines across nodes.
Besides, we plan to retrain, personalize, or optimize models in a pipeline directly on a device,
which may incorporate federated learning~\cite{FederatedLearning}, reinforced learning~\cite{ReinforcedLearning_mnih2013playing}, and partial model updates~\cite{CoreML3_MLUPDATE}.
